The vanishing of strong turbulent fronts in bent pipes

Isolated patches of turbulence in transitional straight pipes are sustained by a strong instability at their upstream front, where the production of turbulent kinetic energy (TKE) is up to five times higher than in the core. Direct numerical simulations presented in this paper show no evidence of such strong fronts if the pipe is bent. We examine the temporal and spatial evolution of puffs and slugs in a toroidal pipe with pipe-to-torus diameter ratio $\delta = D/d = 0.01$ at several subcritical Reynolds numbers. Results show that the upstream overshoot of TKE production is at most one-and-a-half times the value in the core and that the average cross-flow fluctuations at the front are up to three times lower if compared to a straight pipe, while attaining similar values in the core. Localised turbulence can be sustained at smaller energies through a redistribution of turbulent fluctuations and vortical structures by the in-plane Dean motion of the mean flow. This asymmetry determines a strong localisation of TKE production near the outer bend, where linear and nonlinear mechanisms optimally amplify perturbations. We further observe a substantial reduction of the range of Reynolds numbers for long-lived intermittent turbulence, in agreement with experimental data from the literature. Moreover, no occurrence of nucleation of spots through splitting could be detected in the range of parameters considered. Based on the present results, we argue that this mechanism gradually becomes marginal as the curvature of the pipe increases and the transition scenario approaches a dynamical switch from subcritical to supercritical.

==> Makefile <==
#------------------------------------------------------------------------------
# This is a makefile tailored to work on the latex documents for the beamer
# FLOW template.
#------------------------------------------------------------------------------


# Variables:
#
main = manuscript

TEX = pdflatex
TEX_FLAGS =

BIB = bibtex
BIB_FLAGS =


# Dependencies:
#
SRCS = $(main).tex      \
		 abstract.tex     \
		 introduction.tex \
		 spacetimeq.tex   \
		 tkebudget.tex

AUXS = $(main).aux      \
       $(main).toc      \
       $(main).nav      \
       $(main).snm

BBLS = $(main).bbl

# Rules:
#
default: all

all: $(main)
#
$(main): $(SRCS) $(AUXS) $(BBLS)
	@echo building $(main) with $(TEX)
	@$(TEX) $(TEX_FLAGS) -draftmode $(main) #> /dev/null
	@$(TEX) $(TEX_FLAGS) $(main) #> /dev/null

$(AUXS): $(SRCS)
	@echo building $(main) with $(TEX) [for $@]
	@$(TEX) $(TEX_FLAGS) -draftmode $(main) #> /dev/null

%.bbl: %.aux bibliography.bib
	@echo building $@ with $(BIB)
	@$(BIB) $(BIB_FLAGS) $(basename $@) #> /dev/null
#
clean:
	@echo cleaning $(main)
	@rm -f *.ps *.dvi *.aux *.auxlock *.toc *.log *.out *.bbl *.blg *.nav *.snm *~ *.syntex.gz

